Learning Indoor Layouts from Simple Point-Clouds

Reconstructing a layout of indoor spaces has been a crucial part of growing indoor location based services. One of the key challenges in the proliferation of indoor location based services is the unavailability of indoor spatial maps due to the complex nature of capturing an indoor space model (e.g., floor plan) of an existing building. In this paper, we propose a system to automatically generate floor plans that can recognize rooms from the point-clouds obtained through smartphones like Google's Tango. In particular, we propose two approaches - a Recurrent Neural Network based approach using Pointer Network and a Convolutional Neural Network based approach using Mask-RCNN to identify rooms (and thereby floor plans) from point-clouds. Experimental results on different datasets demonstrate approximately 0.80-0.90 Intersection-over-Union scores, which show that our models can effectively identify the rooms and regenerate the shapes of the rooms in heterogeneous environment.

==> xtrash/02-overview.tex <==
\section{Overview}

\begin{figure*}[t!]
    \centering
        \subfloat[Point-cloud of an indoor scene]{\includegraphics[width=0.3\linewidth]{figs/pointcloud-crop.png}}
        \qquad
        \subfloat[Wall detection]{\includegraphics[width=0.3\linewidth]{figs/filtered-hist.pdf}}
        \qquad
        \subfloat[Room detection]{\includegraphics[width=0.3\linewidth]{figs/map.png}}
    \caption{Overview of our system}
    \label{fig:overview}
\end{figure*}

In this section, we briefly describe how our system works and how an user can use our system to map an indoor space. First, the user captures the indoor scene using Google Project Tango API. To capture the scene, he takes the device in hand and walks around the space pointing the Google Tango device towards the wall. Unlike the previous approaches, the user does not necessarily have to capture the scene in detail. With the help of Tango's depth sensing and motion sensing capabilities, a 3D mesh of the indoor scene will be produced. Then, a large number of 3D points are sampled from the 3D mesh. This collection of 3D points, known as a point-cloud (Figure \ref{fig:overview}(a)), is the input of our system.

% \begin{figure*}[h]
%     \centering
%         \subfloat[3D reconstruction using Google Tango API]{\includegraphics[width=0.2\linewidth]{figs/screen-1.jpg}}
%         \qquad
%         \subfloat[Selecting a scene to generate map]{\includegraphics[width=0.2\linewidth]{figs/screen-2.jpg}}
%         \qquad
%         \subfloat[Extracted walls]{\includegraphics[width=0.2\linewidth]{figs/screen-3.jpg}}
%         \qquad
%         \subfloat[Final floor plan]{\includegraphics[width=0.2\linewidth]{figs/screen-4.jpg}}
%     \caption{Screen shots of the whole work-flow of using our system}
%     \label{fig:screen}
% \end{figure*}

After that, we detect the walls by projecting every point onto the floor. This gives us a 2D histogram in a grid like structure containing bins. We only take those bins that contain points more than a certain threshold (this threshold is set from the empirical evaluation). This gives us those bins that contain the walls as shown in Figure \ref{fig:overview}(b). Finally, two different neural networks (Pointer Network and Mask R-CNN) identify the locations of the rooms (Figure \ref{fig:overview}(c)) from the extracted walls. In this study, we consider rooms of different shapes, such as rectangle, rectilinear polygon, room with non-right angles and curved walls.

\endinput
